From Determinism to Delegation: AI-Native Software Engineering and the Evolution of the Agentic Engineer

Software engineering is experiencing its most significant transformation since the emergence of high-level programming languages. As large language models (LLMs) increasingly enable sustained, multi-step, tool-mediated execution, engineering value is shifting from writing deterministic code to supervising probabilistic and autonomous behavior. This paper argues that AI-Native Software Engineering is a paradigm shift rather than a mere tooling advance, creating a new professional archetype: the Agentic Engineer, whose primary artifact is the agentic system rather than the program. We characterize this transition through three changes: (i) the unit of work shifts from functions to supervised agent workflows, (ii) correctness shifts from binary assertions to statistical evaluation under uncertainty, and (iii) accountability shifts from code authorship to outcome ownership. Drawing on post-2022 research, we compare traditional and agentic engineering roles and define core mechanisms of autonomous agents, including reasoning-acting loops, context engineering, tool use, memory, behavioral drift, and compositional error. We place human-AI collaboration within socio-technical frameworks and examine mixed empirical evidence. While some studies report productivity gains, others show slowdowns among experienced developers, highlighting disciplined oversight rather than automation as the critical competency. Using established governance frameworks, we identify required skills and risks, including indirect prompt injection. We conclude that the future is one of symbiosis rather than substitution: agentic engineering builds upon and depends on classical software engineering principles.

==> tables.tex <==
% --- Thematic distribution ---
\begin{table}[ht]
\centering
\caption{Distribution of the 48 verified studies across nine research themes.}
\label{tab:themes}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{p{6.9cm}cc}
\toprule
\textbf{Research theme} & \textbf{\#} & \textbf{\%} \\ \midrule
Foundational Models \& Benchmarks & 6 & 12.5 \\
Agentic \& Multi-Agent SE & 5 & 10.4 \\
SE Task Automation & 2 & 4.2 \\
Code Quality, Security \& Trust & 3 & 6.2 \\
Productivity \& Human-AI Collaboration & 7 & 14.6 \\
Workforce, Labor \& Roles & 6 & 12.5 \\
Computing Education: Capability \& Assessment & 6 & 12.5 \\
Computing Education: Pedagogy \& Tools & 6 & 12.5 \\
Computing Education: Effects \& Adaptation & 3 & 6.2 \\
Synthesis, SLR \& Vision & 4 & 8.3 \\
\midrule
\textbf{Total} & \textbf{48} & \textbf{100.0} \\ \bottomrule
\end{tabular}
\end{table}

% --- Full corpus table (spans multiple pages automatically) ---
\begin{longtable}{c p{4.4cm} c p{2.4cm} c p{5.1cm}}
\caption{Review corpus: 48 studies on LLMs in software engineering and computing education (2016--2026), grouped by theme. Methods: RCT=controlled/field experiment; SUR=survey; QUAL=qualitative/observational; BNCH=benchmark/dataset; TOOL=tool/model+evaluation; SLR=systematic review; POS=position/vision.}
\label{tab:corpus} \\
\toprule
\textbf{ID} & \textbf{Study (cite)} & \textbf{Yr} & \textbf{Venue} & \textbf{Method} & \textbf{Core contribution} \\ \midrule
\endfirsthead

\multicolumn{6}{c}{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\toprule
\textbf{ID} & \textbf{Study (cite)} & \textbf{Yr} & \textbf{Venue} & \textbf{Method} & \textbf{Core contribution} \\ \midrule
\endhead

\midrule \multicolumn{6}{r}{{Continued on next page}} \\ \bottomrule
\endfoot

\bottomrule
\endlastfoot

\multicolumn{6}{l}{\cellcolor{black!8}\textbf{Foundational Models \& Benchmarks}} \\
1 & Codex / HumanEval~\cite{chen2021codex} & 2021 & arXiv & BNCH & Solves 28.8\% of HumanEval at pass@1 (70.2\% at pass@100); repeated sampling sharply boosts solve rate. \\
2 & AlphaCode~\cite{li2022alphacode} & 2022 & Science & TOOL & First system to reach $\sim$top 54\% in simulated Codeforces contests, solving competition-level problems. \\
3 & CodeBERT~\cite{feng2020codebert} & 2020 & EMNLP Find. & TOOL & First bimodal Transformer on NL+code; SOTA on code search and code-to-documentation. \\
4 & CodeT5~\cite{wang2021codet5} & 2021 & EMNLP & TOOL & Identifier-aware pre-training unifies understanding and generation across 8 languages. \\
5 & StarCoder~\cite{li2023starcoder} & 2023 & TMLR & TOOL & Open, governance-aware 15.5B model (8K context, infilling) rivals some closed models. \\
6 & SWE-bench~\cite{jimenez2024swebench} & 2024 & ICLR & BNCH & On 2,294 real GitHub issues, best model solved only $\sim$2\%, exposing the toy-vs-real gap. \\
\multicolumn{6}{l}{\cellcolor{black!8}\textbf{Agentic \& Multi-Agent SE}} \\
7 & ChatDev~\cite{qian2024chatdev} & 2024 & ACL & TOOL & Chat-driven company of role agents produces small software quickly via structured dialogue. \\
8 & MetaGPT~\cite{hong2024metagpt} & 2024 & ICLR & TOOL & Encoding SOPs into role agents cuts cascading hallucination and improves coherence. \\
9 & SWE-agent~\cite{yang2024sweagent} & 2024 & NeurIPS & TOOL & Purpose-built agent-computer interfaces raise autonomous issue-resolution on SWE-bench. \\
10 & ReAct~\cite{yao2023react} & 2023 & ICLR & TOOL & Interleaving reasoning with actions improves task success; underpins tool-using agents. \\
11 & Reflexion~\cite{shinn2023reflexion} & 2023 & NeurIPS & TOOL & Verbal self-reflection stored in memory yields gains across trials, including code tasks. \\
\multicolumn{6}{l}{\cellcolor{black!8}\textbf{SE Task Automation}} \\
12 & LLMs for Program Repair~\cite{xia2023apr} & 2023 & ICSE & TOOL & Applying pre-trained LLMs directly (no fix-training data) surpasses prior repair techniques. \\
13 & TestPilot~\cite{schafer2024testpilot} & 2024 & IEEE TSE & TOOL & Zero-shot JS unit tests reach 70.2\% median statement coverage vs.\ 51.3\% for prior SOTA. \\
\multicolumn{6}{l}{\cellcolor{black!8}\textbf{Code Quality, Security \& Trust}} \\
14 & Asleep at the Keyboard?~\cite{pearce2022asleep} & 2022 & IEEE S\&P & TOOL & $\sim$40\% of 1,689 Copilot programs across MITRE Top-25 CWEs were vulnerable. \\
15 & Insecure Code with AI?~\cite{perry2023insecure} & 2023 & ACM CCS & RCT & AI-assisted users wrote less secure code yet rated it more secure (overconfidence). \\
16 & Reading Between the Lines~\cite{mozannar2024reading} & 2024 & ACM CHI & QUAL & CUPS taxonomy: much developer time goes to verifying/editing suggestions. \\
\multicolumn{6}{l}{\cellcolor{black!8}\textbf{Productivity \& Human-AI Collaboration}} \\
17 & Impact of AI on Productivity~\cite{peng2023impact} & 2023 & arXiv (MSR) & RCT & Copilot users finished an HTTP-server task 55.8\% faster; larger gains for novices. \\
18 & Productivity of Code Completion~\cite{ziegler2022productivity} & 2022 & ACM MAPS & SUR & Acceptance rate predicts perceived productivity better than persistence metrics. \\
19 & Measuring Copilot's Impact~\cite{ziegler2024measuring} & 2024 & CACM & SUR & Across 2,000+ developers, higher acceptance correlates with productivity and flow. \\
20 & Grounded Copilot~\cite{barke2023grounded} & 2023 & OOPSLA & QUAL & Bimodal use: ``acceleration'' (knowing what to write) vs.\ ``exploration''. \\
21 & Expectation vs.\ Experience~\cite{vaithilingam2022expectation} & 2022 & ACM CHI EA & TOOL & Copilot did not improve time/success, yet most preferred it as a starting point. \\
22 & Usability of AI Assistants~\cite{liang2024largescale} & 2024 & ICSE & SUR & Adopted to cut keystrokes/recall syntax; abandoned when output is hard to trust. \\
23 & Early-2025 AI on OSS Devs~\cite{becker2025metr} & 2025 & arXiv (METR) & RCT & Experienced devs $\sim$19\% slower on mature repos yet believed they were faster. \\
\multicolumn{6}{l}{\cellcolor{black!8}\textbf{Workforce, Labor \& Roles}} \\
24 & GenAI in High-Skilled Work~\cite{cui2025effects} & 2025 & Mgmt.\ Science & RCT & Across three firms, Copilot raised completed tasks $\sim$26\%; juniors gained most. \\
25 & Generative AI at Work~\cite{brynjolfsson2023genai} & 2023 & QJE & QUAL & AI assistant raised resolutions/hour 14\% overall, 34\% for novices. \\
26 & Productivity Effects of GenAI~\cite{noy2023experimental} & 2023 & Science & RCT & ChatGPT cut task time $\sim$40\% and raised quality $\sim$18\%; lower performers gained most. \\
27 & GenAI and the Nature of Work~\cite{hoffmann2024nature} & 2024 & HBS WP & TOOL & After Copilot, devs shifted toward core coding away from coordination, persisting $\sim$2 yr. \\
28 & Rapid Adoption of GenAI~\cite{bick2024rapid} & 2024 & NBER WP & SUR & By late 2024, $\sim$23\% of employed U.S.\ workers had used GenAI for work. \\
29 & Toward AI-Native SE (SE 3.0)~\cite{hassan2024se3} & 2024 & ACM TOSEM & POS & Vision of intent-centric development with AI ``teammates'' replacing code-centric work. \\
\multicolumn{6}{l}{\cellcolor{black!8}\textbf{Computing Education: Capability \& Assessment}} \\
31 & The Robots Are Coming (CS1)~\cite{finnieansley2022robots} & 2022 & ACE & BNCH & Codex outperformed most students on CS1 exams, ranking in the top quartile. \\
32 & Will This Be on the Exam? (CS2)~\cite{finnieansley2023cs2} & 2023 & ACE & BNCH & Codex scored top-quartile on CS2 exams; capability extends beyond CS1. \\
33 & Benchmarking ChatGPT/GPT-4~\cite{phung2023benchmarking} & 2023 & ICER & BNCH & GPT-4 beats ChatGPT and nears human tutors, but still lags on grading. \\
34 & LLMs on Beginner Help Requests~\cite{hellas2023exploring} & 2023 & ICER & TOOL & Codex/GPT-3.5 often miss or over-report issues; human guardrails still needed. \\
35 & Copilot on Simple Problems~\cite{wermelinger2023using} & 2023 & SIGCSE TS & QUAL & Solves many simple problems and aids explaining/testing, but is inconsistent. \\
36 & Prompt Engineering for CS1~\cite{denny2023conversing} & 2023 & SIGCSE TS & TOOL & Solves $\sim$half of 166 CS1 problems first try, $\sim$60\% of rest after prompt edits. \\
\multicolumn{6}{l}{\cellcolor{black!8}\textbf{Computing Education: Pedagogy \& Tools}} \\
37 & Auto-Generated Exercises~\cite{sarsa2022automatic} & 2022 & ICER & TOOL & Codex generates novel exercises (with tests) and keyword-steerable explanations. \\
38 & LLM Code Explanations in Class~\cite{macneil2023experiences} & 2023 & SIGCSE TS & SUR & Students engaged with embedded explanations; line-by-line vs.\ high-level valued differently. \\
39 & Student vs.\ LLM Explanations~\cite{leinonen2023comparing} & 2023 & ITiCSE & TOOL & LLM explanations rated more accurate and easier to understand than student ones. \\
40 & Prompt Problems (Promptly)~\cite{denny2024prompt} & 2024 & SIGCSE TS & TOOL & New exercise: students craft prompts to make an LLM produce correct code. \\
41 & CodeHelp~\cite{liffiton2023codehelp} & 2023 & Koli Calling & TOOL & Guard-railed help that avoids giving answers; well received over a 12-week course. \\
42 & AI Code Generators for Novices~\cite{kazemitabaar2023studying} & 2023 & CHI & RCT & Codex improved completion and retention for ages 10--17 without harming later manual work. \\
\multicolumn{6}{l}{\cellcolor{black!8}\textbf{Computing Education: Effects \& Adaptation}} \\
43 & ``It Knows What I Want''~\cite{prather2024weird} & 2024 & ACM TOCHI & QUAL & Identifies novice behaviors (``shepherding,'' ``drifting'') and over-reliance risks. \\
44 & The Widening Gap~\cite{prather2024widening} & 2024 & ICER & QUAL & GenAI sped up strong students but gave strugglers an ``illusion of competence''. \\
45 & From ``Ban It'' to ``Resistance''~\cite{lau2023banit} & 2023 & ICER & QUAL & Instructor stances split between bans and integration; many foresee assessment redesign. \\
\multicolumn{6}{l}{\cellcolor{black!8}\textbf{Synthesis, SLR \& Vision}} \\
30 & LLMs for SE: An SLR~\cite{hou2024llm4se} & 2024 & ACM TOSEM & SLR & Reviews 395 studies (2017--2024), mapping LLMs to SE tasks, data, and challenges. \\
46 & Programming Is Hard~\cite{becker2023programming} & 2023 & SIGCSE TS & POS & Maps opportunities (scaffolding) and challenges (integrity, over-reliance, equity). \\
47 & The Robots Are Here~\cite{prather2023robotshere} & 2023 & ITiCSE-WGR & SUR & Synthesizes 71 articles plus surveys into a roadmap for adapting CS education. \\
48 & Computing Education in GenAI Era~\cite{denny2024computing} & 2024 & CACM & POS & Flagship review of how GenAI reshapes tools, integrity, equity, and open questions. \\
\end{longtable}
